Multi-Scale Simulation of Complex Systems: A Perspective of Integrating Knowledge and Data

Complex system simulation has been playing an irreplaceable role in understanding, predicting, and controlling diverse complex systems. In the past few decades, the multi-scale simulation technique has drawn increasing attention for its remarkable ability to overcome the challenges of complex system simulation with unknown mechanisms and expensive computational costs. In this survey, we will systematically review the literature on multi-scale simulation of complex systems from the perspective of knowledge and data. Firstly, we will present background knowledge about simulating complex system simulation and the scales in complex systems. Then, we divide the main objectives of multi-scale modeling and simulation into five categories by considering scenarios with clear scale and scenarios with unclear scale, respectively. After summarizing the general methods for multi-scale simulation based on the clues of knowledge and data, we introduce the adopted methods to achieve different objectives. Finally, we introduce the applications of multi-scale simulation in typical matter systems and social systems.

==> Tabels/sec6.1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht]
\begin{center}
\begin{tabular}{c|l|l|l}
\hline
\textbf{Categories}                   & \textbf{Method}           & \textbf{Papers}  & \textbf{Application}  \\ \hline
\hline
\multirow{2}{*}{Domain decomposition} & knowledge-driven          & cite{}           &                       \\ \cline{2-4} 
                                      & data-driven               & cite{}           &                       \\ \hline
\multirow{2}{*}{Multigrid method}     & theory-guided             & cite{}           &                       \\ \cline{2-4}
                                      & technique-introduced      & cite{}           &                       \\ \hline
\end{tabular}
\end{center}
\caption{TYPE A}\label{Tab:type-a}
\end{table*}

==> Tabels/sec6.2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht]
\begin{center}
\begin{tabular}{c|l|l|l}
\hline
\textbf{Categories}                                    & \textbf{Method}           & \textbf{Papers}   & \textbf{Application}  \\ \hline
\hline
\multirow{2}{*}{Data-driven}                           & FEA                       & \cite{}           &                       \\ \cline{2-4} 
                                                       & REV                       & \cite{}           &                       \\ \hline
\multirow{2}{*}{Knowledge-driven}                      & NN surrogated DFT         & \cite{}           &                       \\ \cline{2-4}
                                                       & NN surrogated FEA         & \cite{}           &                       \\ \hline
\multirow{2}{*}{Knowledge and data jointly driven}     & NN enhanced FEA           & \cite{}           &                       \\ \cline{2-4}
                                                       & NN enhanced REV           & \cite{}           &                       \\ \hline
\end{tabular}
\end{center}
\caption{TYPE B}\label{Tab:typeb}
\end{table*}

==> Tabels/sec6.3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht]
\begin{center}
\begin{tabular}{c|l|l|l}
\hline
\textbf{Categories}                                    & \textbf{Method}           & \textbf{Papers}   & \textbf{Application}  \\ \hline
\hline
\multirow{2}{*}{Knowledge-driven}                      & Boundary-constraint       & \cite{}           &                       \\ \cline{2-4} 
                                                       & Overlap interaction       & \cite{}           &                       \\ \hline
\multirow{2}{*}{Data-driven}                           & Sampling-based            & \cite{}           &                       \\ \cline{2-4}
                                                       & Fitting-based             & \cite{}           &                       \\ \hline
\end{tabular}
\end{center}
\caption{TYPE C}\label{Tab:typec}
\end{table*}

==> Tabels/sec6_tbl.tex <==
\begin{table}[]
\centering
\setlength{\leftmargini}{0.4cm}
\begin{tabular}{m{2cm} | m{2cm} | m{5cm} | m{6cm} }
\hline
\textbf{Category1} & \textbf{Category2} & \textbf{xxx} & \textbf{Examples and applications} \\ \hline\hline
\multirow{3}{*}{\makecell[c]{Clear\\scales}}   & Type A & 
\begin{itemize}
    \item Domain decomposition~\cite{brooks2009charmm,fish2021mesoscopic,mosser2017reconstruction,yang2018microstructural,wang2019meta,liu2016self,wang2019coarse,mikolov2010recurrent,wu2020recurrent}
    \item Multigrid~\cite{miehe2007multiscale,gravemeier2010algebraic,yushu2020image,dai2019excmg}
\end{itemize}
&  \\ 
                                & Type B & 
\begin{itemize}
    \item Knowledge-driven~\cite{sridhar2016homogenization,ozdemir2008computational,yuan2009multiple}
    \item Data-driven~\cite{allam2018application,le2015computational,xie2018crystal}
    \item Data and knowledge jointly driven~\cite{karniadakis2021physics,hambli2011multiscale,oishi2017computational}
\end{itemize}
&  \\ 
                                & Type C & 
\begin{itemize}
    \item Knowledge-driven~\cite{tao2010nonintrusive,chakraborty2018hyperdynamics,guo2016multi}
    \item Data-driven~\cite{ingolfsson2022machine,bhatia2021machine,han2017deep}
\end{itemize}
&  \\ \hline
\multirow{2}{*}{\makecell[c]{Unclear\\scales}} & Type D & 
\begin{itemize}
    \item Discovering unknown scales~\cite{hoel2013quantifying,hoel2016can,champion2019discovery}(slow scales, linear scale, coarse scale)
    \item Discovering governing equations~\cite{brunton2016discovering,champion2019data,maulik2021reduced}
    %\item Discovering slow variables~\cite{bramburger2020sparse,wehmeyer2018time,noe2013variational,singer2009detecting,perez2013identification}
\end{itemize}
&   \\ 
& Type E & 
\begin{itemize}
    \item Knowledge-driven
    \item Data-driven~\cite{}
\end{itemize}
                                &  \\ \hline
\end{tabular}%
\end{table}

